Differential Diffusion: Giving Each Pixel Its Strength

Diffusion models have revolutionized image generation and editing, producing state-of-the-art results in conditioned and unconditioned image synthesis. While current techniques enable user control over the degree of change in an image edit, the controllability is limited to global changes over an entire edited region. This paper introduces a novel framework that enables customization of the amount of change per pixel or per image region. Our framework can be integrated into any existing diffusion model, enhancing it with this capability. Such granular control on the quantity of change opens up a diverse array of new editing capabilities, such as control of the extent to which individual objects are modified, or the ability to introduce gradual spatial changes. Furthermore, we showcase the framework's effectiveness in soft-inpainting -- the completion of portions of an image while subtly adjusting the surrounding areas to ensure seamless integration. Additionally, we introduce a new tool for exploring the effects of different change quantities. Our framework operates solely during inference, requiring no model training or fine-tuning. We demonstrate our method with the current open state-of-the-art models, and validate it via both quantitative and qualitative comparisons, and a user study. Our code is available at: https://github.com/exx8/differential-diffusion

==> figs/eval/cam_dam_counterexample.tex <==
\newcommand{\mm}{0.16\textwidth}


\begin{figure*}
  \centering
  \begin{tabular}{cc}
    \multirow{2}{*}{Map 1} & \includegraphics[width=0.3\textwidth, frame, valign=c]{imgs/eval/cam_dam_counterexample/circle.jpg} \\
    & \\
    \multirow{2}{*}{Map 2 / Metric} & 
    \begin{tabular}{ccc}
      \toprule
       & {CAM ($\uparrow$)} & {DAM ($\downarrow$)} \\
      \midrule
            \includegraphics[width=\mm, frame]{imgs/eval/cam_dam_counterexample/half_circle.jpg} & \textbf{0.43} & 39.37\\ 
            \includegraphics[width=\mm, frame]{imgs/eval/cam_dam_counterexample/circle_invert.jpg} & -1 & \textbf{0} \\
                        \includegraphics[width=\mm, frame]{imgs/eval/cam_dam_counterexample/triangle3.jpg} & 0.01 & 43.58 \\


      \bottomrule
    \end{tabular}
  \end{tabular}
  \caption{Comparison of CAM and DAM scores of map 1 to three map 2 options.
  %
  %
  %
  %
  }
  %
\label{cam-dam-couterexample}
\end{figure*}


==> figs/eval/spatial_bias.tex <==
\begin{figure}
  \centering
\includegraphics[width=0.15\textwidth,frame]{imgs/eval/spatial_bias.jpg}
\caption{This figure shows the perceptual similarity map's spatial bias.}
\label{fig:spatial_bias}
\end{figure}


==> intro2.tex <==
\section{Introduction}

If you want to edit an image, many options are available.
Besides traditional approaches such as manual editing via Photoshop, modern AI tools are at your service. 
For example, you can edit your image via text instructions~\cite{brooks2023instructpix2pix}.
The most successful image generators that were developed in recent years use a diffusion process \cite{saharia2022palette,rombach2022highresolution},
and in many of these models you can configure the amount of change made to the picture.
But what if you want to edit a region (a specific region of the picture)? In works such as Blended Diffusion~\cite{Avrahami_2022}, you can select which regions of the picture to edit binarily. However, 
it is, at most, a binary choice. 
When you edit a picture, you can only specify 
one amount of change (which is usually termed ``strength''). 
regions of the image are changed by the same strength, or not changed at all.
This is limiting. Sometimes, an editor wishes to change different regions of the image in different amounts. 
For example, if you add mushrooms to a pizza, you might want to add for different slices a different amount of mushrooms. In another example, given a photo of a person, instead of limiting yourself to zombifying the entire person, you might want to zombify different body parts in different amounts, indicating a progressive decaying process.

Furthermore, sometimes the editor wishes to have a continuous transition between adjacent regions. This is sometimes visually more favorable and photo-realistic.  


We present a novel technique for prompt-based image editing, which enables a user to determine the strength of editing each pixel in the image, thus controlling which parts of the image will remain as-is, and which will be changed \emph{and by how much}. Unlike previous methods, we allow the user to choose the quantity of change in a non-binary fashion, thus enabling greater flexibility and finer-grained editing of the image. 
We make key observations (\Cref{observations}) that allow us to create an efficient inference process (\Cref{subsec:region-inject}).
Our technique does not require training or fine-tuning, and it only adds minimal overhead to the inference process~\Cref{peak-vram}.
We demonstrate several applications of our method, and evaluate it against several baselines (\Cref{sec:results}).
Our main contributions are:
\begin{itemize}
    \item We define new methods to manipulate the inference process of diffusion models. See: ~\Cref{subsec:region-inject,hinting}.
    \item We utilize them for creating a new inference process which is capable of editing a picture by different quantities according to a map ---~\Cref{algo}.
    \item We suggested a new metric for comparing different techniques according to their adherents for such maps.
\end{itemize}

